Code2Snapshot: Using Code Snapshots for Learning Representations of Source Code

There are several approaches for encoding source code in the input vectors of neural models. These approaches attempt to include various syntactic and semantic features of input programs in their encoding. In this paper, we investigate Code2Snapshot, a novel representation of the source code that is based on the snapshots of input programs. We evaluate several variations of this representation and compare its performance with state-of-the-art representations that utilize the rich syntactic and semantic features of input programs. Our preliminary study on the utility of Code2Snapshot in the code summarization and code classification tasks suggests that simple snapshots of input programs have comparable performance to state-of-the-art representations. Interestingly, obscuring input programs have insignificant impacts on the Code2Snapshot performance, suggesting that, for some tasks, neural models may provide high performance by relying merely on the structure of input programs.

==> refs_doi.tex <==
%%% Survey
@article{allamanis2018survey,
    title = {A Survey of Machine Learning for Big Code and Naturalness},
    author = {Allamanis, Miltiadis and Barr, Earl T. and Devanbu, Premkumar and Sutton, Charles},
    journal = {{ACM} Computing Surveys},
    volume = {51},
    number = {4},
    year = {2018},
    articleno = {81},
    pages = {1--37},
    numpages = {37},
    doi = {10.1145/3212695},
    url = {https://doi.org/10.1145/3212695}
}

@article{harman2020survey,
    author = {J. M. Zhang and M. Harman and L. Ma and Y. Liu},
    journal = {IEEE Transactions on Software Engineering (TSE)},
    title = {Machine Learning Testing: Survey, Landscapes and Horizons},
    year = {2022},
    volume = {48},
    number = {01},
    issn = {1939-3520},
    pages = {1--36},
    doi = {10.1109/TSE.2019.2962027},
    url = {https://doi.org/10.1109/TSE.2019.2962027}
}

@misc{chen2019embeddings,
    title={A literature study of embeddings on source code},
    author={Chen, Zimin and Monperrus, Martin},
    year={2019},
    doi={10.48550/ARXIV.1904.03061},
    url={https://arxiv.org/abs/1904.03061}
}

@misc{sharma2021survey,
    author={Sharma, Tushar and Kechagia, Maria and Georgiou, Stefanos and Tiwari, Rohit and Sarro, Federica},
    title={A Survey on Machine Learning Techniques for Source Code Analysis},
    year={2021},
    doi={10.48550/ARXIV.2110.09610},
    url={https://arxiv.org/abs/2110.09610}
}

%%% CI
@inproceedings{allamanis2015suggesting,
    author = {Allamanis, Miltiadis and Barr, Earl T. and Bird, Christian and Sutton, Charles},
    title = {Suggesting Accurate Method and Class Names},
    booktitle = {Proceedings of the 10th Joint Meeting on Foundations of Software Engineering (ESEC/FSE)},
    location = {Bergamo, Italy},
    year = {2015},
    pages = {38--49},
    numpages = {12},
    doi = {10.1145/2786805.2786849},
    url = {https://doi.org/10.1145/2786805.2786849}
}

@inproceedings{allamanis2014conventions,
    author = {Allamanis, Miltiadis and Barr, Earl T. and Bird, Christian and Sutton, Charles},
    title = {Learning Natural Coding Conventions},
    booktitle = {Proceedings of the 22nd ACM SIGSOFT International Symposium on Foundations of Software Engineering (FSE)},
    location = {Hong Kong, China},
    year = {2014},
    pages = {281--293},
    numpages = {13},
    doi = {10.1145/2635868.2635883},
    url = {https://doi.org/10.1145/2635868.2635883}
}

@inproceedings{allamanis2016summarization,
    author = {Miltiadis Allamanis and Hao Peng and
    Charles A. Sutton},
    title = {A Convolutional Attention Network for Extreme Summarization of Source Code},
    booktitle = {Proceedings of the 33nd International Conference on Machine Learning (ICML)},
    location = {New York, NY, USA},
    year = {2016},
    pages = {2091--2100},
    numpages = {10},
    url = {http://proceedings.mlr.press/v48/allamanis16.html}
}

@article{alon2019code2vec,
    author = {Alon, Uri and Zilberstein, Meital and Levy, Omer and Yahav, Eran},
    title = {code2vec: Learning Distributed Representations of Code},
    journal = {Proceedings of the {ACM} on Programming Languages (PACMPL)},
    volume = {3},
    number = {POPL},
    year = {2019},
    issn = {2475-1421},
    pages = {40:1--40:29},
    articleno = {40},
    numpages = {29},
    url = {http://doi.acm.org/10.1145/3290353},
    doi = {10.1145/3290353},
}

@inproceedings{alon2019code2seq,
    title={code2seq: Generating Sequences from Structured Representations of Code},
    author={Uri Alon and Omer Levy and Eran Yahav},
    booktitle={The 7th International Conference on Learning Representations (ICLR)},
    year={2019},
    url={https://openreview.net/forum?id=H1gKYo09tX},
}

@inproceedings{allamanis2018ggnn,
    title={Learning to Represent Programs with Graphs},
    author={Miltiadis Allamanis and Marc Brockschmidt and Mahmoud Khademi},
    booktitle={The 6th International Conference on Learning Representations (ICLR)},
    year={2018},
    url={https://openreview.net/forum?id=BJOFETxR-},
}

@inproceedings{hellendoorn2018type,
    author = {Hellendoorn, Vincent J. and Bird, Christian and Barr, Earl T. and Allamanis, Miltiadis},
    title = {Deep Learning Type Inference},
    year = {2018},
    url = {https://doi.org/10.1145/3236024.3236051},
    doi = {10.1145/3236024.3236051},
    booktitle = {Proceedings of the 26th ACM Joint Meeting on European Software Engineering Conference and Symposium on the Foundations of Software Engineering (ESEC/FSE)},
    pages = {152--162},
    location = {Lake Buena Vista, FL, USA},
}

%%% Do
@inproceedings{compton2020obfuscation,
    author = {Compton, Rhys and Frank, Eibe and Patros, Panos and Koay, Abigail},
    title = {Embedding Java Classes with Code2vec: Improvements from Variable Obfuscation},
    booktitle = {Proceedings of the 17th International Conference on Mining Software Repositories (MSR)},
    location = {Seoul, Republic of Korea},
    year = {2020},
    pages = {243--253},
    numpages = {11},
    doi = {10.1145/3379597.3387445},
    url = {https://doi.org/10.1145/3379597.3387445}
}

@inproceedings{suneja2020probing,
    author = {Suneja, Sahil and Zheng, Yunhui and Zhuang, Yufan and Laredo, Jim A. and Morari, Alessandro},
    title = {Probing Model Signal-Awareness via Prediction-Preserving Input Minimization},
    booktitle = {Proceedings of the 29th ACM Joint Meeting on European Software Engineering Conference and Symposium on the Foundations of Software Engineering (ESEC/FSE)},
    location = {Athens, Greece},
    year = {2021},
    pages = {945--955},
    numpages = {11},
    doi = {10.1145/3468264.3468545},
    url = {https://doi.org/10.1145/3468264.3468545}
}

@inproceedings{allamanis2019duplication,
    author = {Allamanis, Miltiadis},
    title = {The Adverse Effects of Code Duplication in Machine Learning Models of Code},
    year = {2019},
    booktitle = {Proceedings of the ACM SIGPLAN International Symposium on New Ideas, New Paradigms, and Reflections on Programming and Software (Onward!)},
    pages = {143--153},
    numpages = {11},
    location = {Athens, Greece},
    doi = {10.1145/3359591.3359735},
    url = {https://doi.org/10.1145/3359591.3359735},
}

@inproceedings{bui2019sa,
    author={Bui, Nghi D. Q. and Yu, Yijun and Jiang, Lingxiao},
    title={Bilateral Dependency Neural Networks for Cross-Language Algorithm Classification},
    booktitle={Proceedings of the 26th IEEE International Conference on Software Analysis, Evolution and Reengineering (SANER)},
    year={2019},
    volume={},
    number={},
    pages={422-433},
    doi={10.1109/SANER.2019.8667995}
}

%%% CNN
@article{krizhevsky2012alexnet,
    author = {Krizhevsky, Alex and Sutskever, Ilya and Hinton, Geoffrey E.},
    title = {ImageNet Classification with Deep Convolutional Neural Networks},
    year = {2017},
    volume = {60},
    number = {6},
    issn = {0001-0782},
    url = {https://doi.org/10.1145/3065386},
    doi = {10.1145/3065386},
    journal = {Communications of the {ACM}},
    pages = {84--90},
    numpages = {7}
}

@inproceedings{he2016resnet,
    author={He, Kaiming and Zhang, Xiangyu and Ren, Shaoqing and Sun, Jian},
    booktitle={Proceedings of the 29th IEEE Conference on Computer Vision and Pattern Recognition (CVPR)}, 
    title={Deep Residual Learning for Image Recognition}, 
    year={2016},
    volume={},
    number={},
    pages={770--778},
    doi={10.1109/CVPR.2016.90},
    url={https://doi.org/10.1109/CVPR.2016.90},
}

@inproceedings{zeiler2014visualizing,
    author="Zeiler, Matthew D.
    and Fergus, Rob",
    editor="Fleet, David
    and Pajdla, Tomas
    and Schiele, Bernt
    and Tuytelaars, Tinne",
    title="Visualizing and Understanding Convolutional Networks",
    booktitle="Proceedings of the 13th European Conference on Computer Vision (ECCV)",
    year="2014",
    pages="818--833",
}

@inproceedings{selvaraju2017grad,
  title={Grad-cam: Visual explanations from deep networks via gradient-based localization},
  author={Selvaraju, Ramprasaath R and Cogswell, Michael and Das, Abhishek and Vedantam, Ramakrishna and Parikh, Devi and Batra, Dhruv},
  booktitle={Proceedings of the 18th IEEE International Conference on Computer Vision (ICCV)},
  pages={618--626},
  year={2017},
  doi={10.1109/ICCV.2017.74},
  url={https://doi.org/10.1109/ICCV.2017.74},
}

%%% Image
@article{dey2019socodecnn,
  title={{SoCodeCNN}: Program source code for visual {CNN} classification using computer vision methodology},
  author={Dey, Somdip and Singh, Amit Kumar and Prasad, Dilip Kumar and Mcdonald-Maier, Klaus Dieter},
  journal={IEEE Access},
  volume={7},
  pages={157158--157172},
  year={2019},
  doi={10.1109/ACCESS.2019.2949483},
  url={https://doi.org/10.1109/ACCESS.2019.2949483},
}

@article{keller2020visualization,
    author = {Keller, Patrick and Kabor\'{e}, Abdoul Kader and Plein, Laura and Klein, Jacques and Le Traon, Yves and Bissyand\'{e}, Tegawend\'{e} F.},
    title = {What You See is What It Means! Semantic Representation Learning of Code Based on Visualization and Transfer Learning},
    year = {2021},
    volume = {31},
    number = {2},
    issn = {1049-331X},
    url = {https://doi.org/10.1145/3485135},
    doi = {10.1145/3485135},
    journal={ACM Transactions on Software Engineering and Methodology (TOSEM)},
    articleno = {31},
    numpages = {34}
}

@misc{bilgin2021code2image,
  doi = {10.48550/ARXIV.2105.03131},
  url = {https://arxiv.org/abs/2105.03131},
  author = {Bilgin, Zeki},
  title = {Code2Image: Intelligent Code Analysis by Computer Vision Techniques and Application to Vulnerability Prediction},
  year = {2021},
}

%%% Tool

@misc{clark2019pil,
  author = {Alex Clark and Contributors},
  title = {{Pillow (Fork of the Python Imaging Library)}},
  howpublished = "\url{https://github.com/python-pillow/Pillow/}",
  year={2021},
  note = "[Online; accessed 31-July-2021]"
}

@misc{pil,
  author = {{Alex Clark and Contributors}},
  title = {{Pillow (Fork of the Python Imaging Library)}},
  howpublished = "\url{https://github.com/python-pillow/Pillow/}",
  year={2010},
  note = "[Online; accessed 31-July-2021]"
}

@misc{javaparser,
  author = {{Danny van Bruggen and Contributors}},
  title = {{JavaParser (Tools for Java code)}},
  howpublished = "\url{https://github.com/javaparser/javaparser/}",
  year={2011},
  note = "[Online; accessed 31-July-2021]"
}

%%% rabin
@article{rabin2019tnpa,
    title={Testing Neural Program Analyzers},
    author={Rabin, Md Rafiqul Islam and  Wang, Ke and Alipour, Mohammad Amin},
    journal={IEEE/ACM International Conference on Automated Software Engineering: Late Breaking Results (ASE-LBR)},
    year={2019},
    doi={10.48550/arXiv.1908.10711},
    url={https://doi.org/10.48550/arXiv.1908.10711}
}

@inproceedings{rabin2020demystifying,
    author = {Rabin, Md Rafiqul Islam and Mukherjee, Arjun and Gnawali, Omprakash and Alipour, Mohammad Amin},
    title = {Towards Demystifying Dimensions of Source Code Embeddings},
    booktitle = {Proceedings of the 1st ACM SIGSOFT International Workshop on Representation Learning for Software Engineering and Program Languages (RL+SE\&PL)},
    location = {Virtual, USA},
    year = {2020},
    pages = {29--38},
    numpages = {10},
    doi = {10.1145/3416506.3423580},
    url = {https://doi.org/10.1145/3416506.3423580}
}

@article{rabin2021generalizability,
    author = {Md Rafiqul Islam Rabin and Nghi D.Q. Bui and Ke Wang and Yijun Yu and Lingxiao Jiang and Mohammad Amin Alipour},
    title = {On the generalizability of Neural Program Models with respect to semantic-preserving program transformations},
    journal = {Information and Software Technology (IST)},
    volume = {135},
    year = {2021},
    pages = {106552},
    doi = {https://doi.org/10.1016/j.infsof.2021.106552},
    url = {https://www.sciencedirect.com/science/article/pii/S0950584921000379}
}

@inproceedings{rabin2021sivand,
    author = {Rabin, Md Rafiqul Islam and Hellendoorn, Vincent J. and Alipour, Mohammad Amin},
    title = {Understanding Neural Code Intelligence through Program Simplification},
    booktitle = {Proceedings of the 29th ACM Joint Meeting on European Software Engineering Conference and Symposium on the Foundations of Software Engineering (ESEC/FSE)},
    location = {Athens, Greece},
    year = {2021},
    pages = {441--452},
    numpages = {12},
    doi = {10.1145/3468264.3468539},
    url = {https://doi.org/10.1145/3468264.3468539}
}

@inproceedings{rabin2022perses,
    author = {Rabin, Md Rafiqul Islam and Hussain, Aftab and Alipour, Mohammad Amin},
    title = {Syntax-Guided Program Reduction for Understanding Neural Code Intelligence Models},
    booktitle = {Proceedings of the 6th Annual Symposium on Machine Programming (MAPS)},
    location = {San Diego, California, United States},
    year = {2022},
    pages = {},
    numpages = {},
    doi = {10.1145/3520312.3534869},
    url = {https://doi.org/10.1145/3520312.3534869}
}

@misc{rabin2021memorization,
    title={Memorization and Generalization in Neural Code Intelligence Models}, 
    author={Md Rafiqul Islam Rabin and Aftab Hussain and Mohammad Amin Alipour and Vincent J. Hellendoorn},
    year={2021},
    eprint={2106.08704},
    archivePrefix={arXiv},
    primaryClass={cs.LG},
    url = {https://arxiv.org/abs/2106.08704}
}

%%% Unknown
@inproceedings{DeFreez,
    author = {DeFreez, Daniel and Thakur, Aditya V. and Rubio-Gonz\'{a}lez, Cindy},
    title = {Path-based Function Embeddings},
    booktitle = {Proceedings of the 40th International Conference on Software Engineering (ICSE)},
    year = {2018},
    location = {Gothenburg, Sweden},
    pages = {430--431},
    numpages = {2},
    url = {http://doi.acm.org/10.1145/3183440.3195042},
    doi = {10.1145/3183440.3195042},
} 


==> validity.tex <==
\section{Threats to Validity}

We have only evaluated the \approach embeddings for code summarization task on the most frequent labels. Despite our best effort, it is possible that experiments with different models, sizes of images, and font settings may produce different results. Our further plan also includes a detailed study with a variety of code intelligence tasks, embeddings, and datasets.

